Propagation and Decay of Injected One-Off Delays on Clusters: A Case Study

Analytic, first-principles performance modeling of distributed-memory applications is difficult due to a wide spectrum of random disturbances caused by the application and the system. These disturbances (commonly called "noise") destroy the assumptions of regularity that one usually employs when constructing simple analytic models. Despite numerous efforts to quantify, categorize, and reduce such effects, a comprehensive quantitative understanding of their performance impact is not available, especially for long delays that have global consequences for the parallel application. In this work, we investigate various traces collected from synthetic benchmarks that mimic real applications on simulated and real message-passing systems in order to pinpoint the mechanisms behind delay propagation. We analyze the dependence of the propagation speed of idle waves emanating from injected delays with respect to the execution and communication properties of the application, study how such delays decay under increased noise levels, and how they interact with each other. We also show how fine-grained noise can make a system immune against the adverse effects of propagating idle waves. Our results contribute to a better understanding of the collective phenomena that manifest themselves in distributed-memory parallel applications.

==> figures/Pi_TRIAD_strongscaling/README <==
Showcase experiment for deviation in model:

Downscaling runtime vs. number of nodes graph using homogeneous situation and strong scaling (increase number of nodes with same problem (same problem size with constant communication overhead))

In contrast to model expectation: performance better as computation time goes down with increase in number of nodes gives decline curve and non-ideal speedup

Example that show model as lower-bound: Triad results even better than pi

Note1: contention (network/memory) gives you even more better results
Note2: all values in text files are in ms

device = EMMY 				#    key value for CPU device
ppn		= 1, 20				# 	 (a int) the number of processes per node
numDirShifts = 2			#	 (a int) number of direction of shifts in each dimension ( 1: uni-directional upwards shift [only positive direction], 2: bi-directional upwards and downwards shift [both positive and negative directions]) 
ShiftStep	 = 1			#	 (a int) step size of shifts in each dimension
periodicX 	 = 1			#	 (a bool) periodic (true=1) or non-periodic (false=0) in x dimension

# memory-bound stream triad benchmark 
arraySize 	 = 50000000	#	 (a int) Default array size (number of elements per array)
scalar 		 = 0.41			#    (a int) scalar coefficient value
arrayAlignment = 64	    	#	 (a int) It provides partial support for adjusting relative alignment

# communication-related information
msgSizeBytes 	 =   2000000	#	  (a int) Message size (number of doubles)

# /**
#	* \brief timing-specific information
# */
numTimeStep  = 1000			#  (a int) Outer iteration count, i.e., N loops of T seconds = N * T seconds 
timingRep 	 = 10			#	 (a int) repetion count of C++ high resolution clock timing measurements to take average in the end



